Fine-Grained Prediction of Reading Comprehension from Eye Movements

Can human reading comprehension be assessed from eye movements in reading? In this work, we address this longstanding question using large-scale eyetracking data over textual materials that are geared towards behavioral analyses of reading comprehension. We focus on a fine-grained and largely unaddressed task of predicting reading comprehension from eye movements at the level of a single question over a passage. We tackle this task using three new multimodal language models, as well as a battery of prior models from the literature. We evaluate the models' ability to generalize to new textual items, new participants, and the combination of both, in two different reading regimes, ordinary reading and information seeking. The evaluations suggest that although the task is highly challenging, eye movements contain useful signals for fine-grained prediction of reading comprehension. Code and data will be made publicly available.

==> notes.tex <==
%%%%%%%%%% 
% References for foundation models with multimodal question answering capabilities
%%%%%%%%%%%
%Recently,  the rise of so-called \textit{foundational models} \tbdref has led to multimodal integration directions that make use of such models, while not requiring fine-tuning the full model \cite{luo_cheap_2023,liu_visual_2023} in general and for multimodal question answering \cite{zhang_pmc-vqa_2023-1,zhang_finetuning_2023,he_pefomed_2024} specifically. Typical modalities in addition to text are vision (i.e. images/videos) and auditory (voices/sounds).




%Makowsky: chance level results on a binary task aggregating responses across 3 questions over each text

%Our work addresses comprehension prediction at the granularity of an individual question over a paragraph, and includes systematic model evaluation across different evaluation regimes. It further introduces key innovations over prior work on prediction of reading comprehension. Importantly, we extend the standard correct versus incorrect distinction to prediction of specific distractors. The STARC annotation framework \cite{berzak-2020-starc} discussed in Section \ref{data-and-annotations}, %classifies answer selections in a 4-tier hierarchy of comprehension and ties them to their textual support, 
%allows us to further analyze specific incorrect responses according to degree of text comprehension. Our study also builds on comparative analyses of eye movements in ordinary and information seeking reading \cite{hahnkeller2023,shubi2023cogsci} to systematically examine the effects of ordinary versus goal oriented reading. Taken together, these aspects constitute a more fine-grained characterization of the ability to predict reading comprehension from gaze than previously possible.

%Differences from prior work
%\begin{itemize}
%\item paragraph level (as opposed to sentence level, or article level)
%\item q immediately after reading p
%\item differently from \cite{}, separation between paragraph reading and qa
%\item key: In \citet{Ahn2020SBSAT} and \citet{ReichETRA2022} aggregation of responses across reading comprehension items and binning to low (below median) versus high (above median) comprehension. Our work does not take these simplifying steps. 
%\item key: go beyond the correct / incorrect distinction to a 4-tier model of understanding
%\item key: characterizing the relation between answers and eye movements over their textual support
%\item key: data at a larger scale than existing datasets, both in terms of number of questions and number of: SB-SAT \citep{Ahn2020SBSAT} has 4 texts (22 paragraphs), 20 questions (5 questions per paragraph) and 95 participants. OneStopQA has an order of magnitude more texts 
%\end{itemize}

%\citet{ReichETRA2022} eval: new text and new reader but not both.
%\citet{meziere2023using} 79 participants, 3 tests. Prediction task: total comprehension score in the test. 
%\begin{itemize}
%    \item YARC (silent reading): 2 paragraphs (over 4 screens, not clear of each or both), 13 open ended questions after each paragraph. Can go back and forth between questions and paragraph. Total score over 13 questions.
%    \item GORT-5 (reading aloud): 16 (possibly only 11?) paragraphs (each 1-3 pages), 5 open ended questions. Cannot go backward while reading. Total 55? questions.
%    \item WRAT-4 (silent reading): 30 items (each 1-2 sentences), missing word (cloze) task.   
%    \item only fixation features. eval old participant old item.
%\end{itemize}

%\citet{copeland2013measuring}
%\citet{copeland2014} 39 participants 
%\begin{itemize}
%    \item 9 paragraphs (each paragraph on a single page), 18 questions (2 questions per paragraph, %one multiple choice 1 close with 3 possible scores 0, 0.5, 1).
%    \item 4 different presentation modes for questions and paragraphs
%    \item item level predictions, above chance results
%    \item only fixation features
%    \item eval: same text old and new participants, poor generalization to new participants.
%\end{itemize}

%\citet{martinez2014} 39 participants
%\begin{itemize}
%    \item 6 documents (1 page each), 8 question each 48 in total.
%    \item prediction of aggregate score (z-scored) for each document, and a binarized version thereof. Above chance only on binarized version.
%    \item both fixation and ling features
%    \item eval: 
%\end{itemize}

%\citet{inhoff2018} comprehension ability is assessed on other sentences, so ok not to cite.

%\citet{southwell2020} 3 experiments (with different manipulations, pooled participants across conditions), Ns = 104, 130, 147, total 381
%\begin{itemize}
%    \item only eye movement features
%    \item eval: same texts, new participants. Average across all items.
%    \item significant correlations found for all 3 datasets
%\end{itemize}
% We evaluated model accuracy by correlating each participant's observed comprehension, averaged across pages (Datasets 1 and 2) or texts (Dataset 3), with their similarly averaged predicted “correct” comprehension class probability (for Datasets 1 and 2 using logistic regression) or predicted comprehension score (Dataset 3 using linear regression). This metric indicates how much between-participant variability in comprehension is captured by the model. Correlations were compared between models using tests of dependent correlations as implemented in the cocor package (Diedenhofen & Musch, 2015).
